The LDBC Financial Benchmark

The Linked Data Benchmark Council's Financial Benchmark (LDBC FinBench) is a new effort that defines a graph database benchmark targeting financial scenarios such as anti-fraud and risk control. The benchmark has one workload, the Transaction Workload, currently. It captures OLTP scenario with complex, simple read queries and write queries that continuously insert or delete data in the graph. Compared to the LDBC SNB, the LDBC FinBench differs in application scenarios, data patterns, and query patterns. This document contains a detailed explanation of the data used in the LDBC FinBench, the definition of transaction workload, a detailed description for all queries, and instructions on how to use the benchmark suite.

==> choke-points/cp-4-4.tex <==
\tpcCPSection{4.4}{QEXE}{String matching performance}

This choke point tests the ability of efficiently evaluating complex string
matching expressions (\eg via regular expressions).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\IfFileExists{choke-point-query-mapping/cp-4-4}{\input{choke-point-query-mapping/cp-4-4}}{}


==> templates/choke-point-query-mapping-template.tex <==
\paragraph{Queries}
{\raggedright
{% for query in queries -%}
    \queryRefCard{ {{- query.0 -}} }{
      {%- if query.1 == "Transaction" and query.2 == "complex-read" -%}
        TCR
      {%- elif query.1 == "Transaction" and query.2 == "simple-read" -%}
        TSR
      {%- elif query.1 == "Transaction" and query.2 == "write" -%}
        TW
      {%- elif query.1 == "Transaction" and query.2 == "read-write" -%}
        TRW
      {%- endif -%}
    }{ {{- query.3 -}} }
{% endfor -%}
{# this newline is required by \raggedright to work #}
}


==> templates/query-card-template.tex <==
\renewcommand*{\arraystretch}{1.1}

\subsection*{ {{- workload }} / {{ operation }} / {{ number -}} }
\label{sec: {{- query_id -}} }

% change \emph{} to use sans-serif font
\let\oldemph\emph
\renewcommand{\emph}[1]{{ '{{' }}\footnotesize \sf #1}}
\let\oldtextbf\textbf
\renewcommand{\textbf}[1]{{ '{{' }}\it #1}}

{%- if workload == "Transaction" and operation == "complex-read" -%}
\renewcommand{\currentQueryCard}{ {{- number -}} }
\marginpar{
	\raggedleft
	\scriptsize
	% \vspace{0.15ex}

	\queryRefCard{transaction-complex-read-01}{TCR}{1}\\
	\queryRefCard{transaction-complex-read-02}{TCR}{2}\\
	\queryRefCard{transaction-complex-read-03}{TCR}{3}\\
	\queryRefCard{transaction-complex-read-04}{TCR}{4}\\
	\queryRefCard{transaction-complex-read-05}{TCR}{5}\\
	\queryRefCard{transaction-complex-read-06}{TCR}{6}\\
	\queryRefCard{transaction-complex-read-07}{TCR}{7}\\
	\queryRefCard{transaction-complex-read-08}{TCR}{8}\\
	\queryRefCard{transaction-complex-read-09}{TCR}{9}\\
	\queryRefCard{transaction-complex-read-10}{TCR}{10}\\
	\queryRefCard{transaction-complex-read-11}{TCR}{11}\\
	\queryRefCard{transaction-complex-read-12}{TCR}{12}\\
	% \queryRefCard{transaction-complex-read-13}{TCR}{13}\\
	% \queryRefCard{transaction-complex-read-14}{TCR}{14}\\
}
{%- endif %}

{%- if workload == "Transaction" and operation == "simple-read" -%}
\renewcommand{\currentQueryCard}{ {{- number -}} }
\marginpar{
	\raggedleft
	\scriptsize
	% \vspace{0.15ex}

	\queryRefCard{transaction-simple-read-01}{TSR}{1}\\
	\queryRefCard{transaction-simple-read-02}{TSR}{2}\\
	\queryRefCard{transaction-simple-read-03}{TSR}{3}\\
	\queryRefCard{transaction-simple-read-04}{TSR}{4}\\
	\queryRefCard{transaction-simple-read-05}{TSR}{5}\\
	\queryRefCard{transaction-simple-read-06}{TSR}{6}\\
	% \queryRefCard{transaction-simple-read-07}{TSR}{7}\\
	% \queryRefCard{transaction-simple-read-08}{TSR}{8}\\
}
{%- endif %}

{%- if workload == "Transaction" and operation == "write" -%}
\renewcommand{\currentQueryCard}{ {{- number -}} }
\marginpar{
	\raggedleft
	\scriptsize
	% \vspace{0.15ex}
	
	\queryRefCard{transaction-write-01}{TW}{1}\\
	\queryRefCard{transaction-write-02}{TW}{2}\\
	\queryRefCard{transaction-write-03}{TW}{3}\\
	\queryRefCard{transaction-write-04}{TW}{4}\\
	\queryRefCard{transaction-write-05}{TW}{5}\\
	\queryRefCard{transaction-write-06}{TW}{6}\\
	\queryRefCard{transaction-write-07}{TW}{7}\\
	\queryRefCard{transaction-write-08}{TW}{8}\\
	\queryRefCard{transaction-write-09}{TW}{9}\\
	\queryRefCard{transaction-write-10}{TW}{10}\\
	\queryRefCard{transaction-write-11}{TW}{11}\\
	\queryRefCard{transaction-write-12}{TW}{12}\\
	\queryRefCard{transaction-write-13}{TW}{13}\\
	\queryRefCard{transaction-write-14}{TW}{14}\\
	\queryRefCard{transaction-write-15}{TW}{15}\\
	\queryRefCard{transaction-write-16}{TW}{16}\\
	\queryRefCard{transaction-write-17}{TW}{17}\\
	\queryRefCard{transaction-write-18}{TW}{18}\\
	\queryRefCard{transaction-write-19}{TW}{19}\\
}
{%- endif %}

{%- if workload == "Transaction" and operation == "read-write" -%}
\renewcommand{\currentQueryCard}{ {{- number -}} }
\marginpar{
	\raggedleft
	\scriptsize
	% \vspace{0.15ex}
	
	\queryRefCard{transaction-read-write-01}{TRW}{1}\\
	\queryRefCard{transaction-read-write-02}{TRW}{2}\\
	\queryRefCard{transaction-read-write-03}{TRW}{3}\\
}
{%- endif %}

\noindent\begin{tabularx}{\queryCardWidth}{|>{\queryPropertyCell}p{\queryPropertyCellWidth}|X|}
	\hline
	query & {{ workload }} / {{ operation }} / {{ number }} \\ \hline
%
	title & {{ title }} \\ \hline
%
	{% if operation == "complex-read" or operation == "simple-read" or operation == "write" or operation == "read-write" %}
		pattern & \centering \includegraphics[scale=\yedscale,margin=0cm .2cm]{patterns/{{ query_id -}} } \tabularnewline \hline
	{% endif %}
%
	{% if composition %}
		compose. & 
		This read-write query contains the reads and writes below,
		\begin{itemize}
			{% for entry in composition -%}
				\item \hyperref[sec:{{ entry.ref }}] { {{ entry.name }} }
			{% endfor -%} 
		\end{itemize}
		\\ \hline
	{% endif %}
%
	desc. & {{ description }} \\ \hline
%
	{% if parameters %}
		params &
		\innerCardVSpace{\begin{tabularx}{\attributeCardWidth}{|>{\paramNumberCell}C{\attributeNumberWidth}|>{\varNameCell}M|>{\typeCell}m{\typeWidth}|Y|} \hline
		{% for entry in parameters -%}
			$\mathsf{ {{- loop.index -}} }$ & {{ entry.name }} & {{ entry.type }} & {{ entry.description }} \\ \hline
		{% endfor -%}
		\end{tabularx}}\innerCardVSpace \\ \hline
	{% endif %}
%
	{% if result %}
		result &
		\innerCardVSpace{\begin{tabularx}{\attributeCardWidth}{|>{\resultNumberCell}C{\attributeNumberWidth}|>{\varNameCell}M|>{\typeCell}m{\typeWidth}|>{\resultOriginCell}c|Y|} \hline
		{% for entry in result -%}
			$\mathsf{ {{- loop.index -}} }$ & {{ entry.name|trim() }} & {{ entry.type|trim() }} & {% set cat = entry.category|trim() -%}
					{%- if   cat == "aggregated" -%} A
					{%- elif cat == "calculated" -%} C
					{%- elif cat == "meta" -%} M
					{%- elif cat == "structural" -%} S
					{%- else -%} R
					{%- endif %} &
				{{ entry.description }} \\ \hline
		{% endfor -%}
		\end{tabularx}}\innerCardVSpace \\ \hline
	{% endif %}
%
	{% if groupby %}
		groupby 	&	{{ groupby }} \\ \hline
	{% endif -%}
%
	{% if sort %}
		sort		&
		\innerCardVSpace{\begin{tabularx}{\attributeCardWidth}{|>{\sortNumberCell}C{\attributeNumberWidth}|>{\varNameCell}X|>{\directionCell}c|Y|} \hline
		{% for entry in sort -%}
			$\mathsf{ {{- loop.index -}} }$ & {{ entry.name }} & $\{{ entry.direction }}$ & {{ entry.description }} \\ \hline
		{% endfor -%}
		\end{tabularx}}\innerCardVSpace \\ \hline
	{% endif -%}
%
	{% if limit -%}
		limit & {{ limit }} \\ \hline
	{% endif -%}
%
	{% if choke_points -%}
	CPs &
	\multicolumn{1}{>{\raggedright}l|}{
		{% for choke_point in choke_points -%}
			\chokePoint{ {{- choke_point -}} } {%- if not loop.last %}, {% endif %}
		{% endfor -%}
	} \\ \hline
	{% endif -%}
%
	% {% if relevance -%}
	% relevance &
	% 	\footnotesize {{ relevance }} \\ \hline
	% {%- endif -%}
%
\end{tabularx}
\queryCardVSpace

% change \emph and \textbf back to the old ones
\let\emph\oldemph
\let\textbf\oldtextbf

\renewcommand{\currentQueryCard}{0}

